Ergodicity and synchronization of the Kardar-Parisi-Zhang equation

The Kardar-Parisi-Zhang (KPZ) equation on the real line is well-known to admit Brownian motion with a linear drift as a stationary distribution (modulo additive constants). We show that these solutions are attractive, a result known as a one force--one solution (1F1S) principle or synchronization: the solution to the KPZ equation started in the distant past from an initial condition with a given slope will converge almost surely to a Brownian motion with that drift, which shows in particular that these invariant measures are totally ergodic. Our proof constructs the Busemann process for the equation, which gives the natural jointly stationary coupling of all of these stationary solutions. Synchronization then holds simultaneously (on a single full probability event) for all but an at most countable random set of asymptotic slopes. This set of exceptional slopes of instability for which synchronization fails is either almost surely empty or almost surely dense. Along the way, we prove a shape theorem which implies almost sure stochastic homogenization of the KPZ equation, for which the Busemann process gives the process of correctors. We also show that the forward and backward point-to-point and point-to-line continuum polymers converge to semi-infinite continuum polymers whose transitions are Doob transforms via Busemann functions of the transitions of the finite length polymers.

==> SHE-macros.tex <==
\newcommand\bmmax{0}
\newcommand\hmmax{0}

\usepackage{amsmath,amsthm,amssymb,tikz,tikz-cd,mathrsfs,pgfplots}
%\usepackage{showkeys}
\usepackage[numbers,comma,square,sort&compress]{natbib}
%\usepackage{enumerate}

\usepackage{rotating,centernot,cancel}    %% to manipulate symbols 

%\usepackage{skull}
%\usepackage{halloweenmath}
%\usepackage{arev}
\usepackage{mathabx}
%\usepackage{bclogo}

\usepackage{enumitem}
%% how to enumerate:  \begin{enumerate}  [label={\rm(\roman*)}, ref={\rm\roman*}]   \itemsep=3pt  
%%% types of  labels:  [label=(roman*)]  \arabic*  \alph*    also under \itemize can use different symbols to mark items

%\usepackage{arevmath}

\usepackage{datetime2}

\RequirePackage{xcolor}
\definecolor{my-link}{rgb}{0.5,0.0,0.0}
\definecolor{my-blue}{rgb}{0.0,0.0,0.6}
\definecolor{my-red}{rgb}{0.5,0.0,0.0}
\definecolor{my-green}{rgb}{0.2,0.5,0.2}
\definecolor{nicos-red}{rgb}{0.75,0.0,0.0}
\definecolor{really-light-gray}{gray}{0.8}
\definecolor{darkgreen}{rgb}{0.0,0.5,0.0}
\definecolor{darkblue}{rgb}{0.0,0.0,0.3}
\definecolor{nicosred}{rgb}{0.65,0.1,0.1}
\definecolor{light-gray}{gray}{0.7}
\RequirePackage[colorlinks,urlcolor=my-blue,linkcolor=my-red,citecolor=my-green]{hyperref}

\usepackage{xargs}
\usepackage[colorinlistoftodos,prependcaption,textsize=footnotesize]{todonotes}
\newcommandx{\addmath}[2][1=]{\todo[linecolor=red,backgroundcolor=red!25,bordercolor=red,#1]{#2}}
\newcommandx{\fixtext}[2][1=]{\todo[linecolor=blue,backgroundcolor=blue!25,bordercolor=blue,#1]{#2}}
\newcommandx{\note}[2][1=]{\todo[linecolor=yellow,backgroundcolor=yellow!25,bordercolor=yellow,#1]{#2}}
\def\timonote#1{{\color{my-green}{(T: #1)}}}
\def\chrisnote#1{{\color{my-blue}{(C: #1)}}}
\def\firasnote#1{{\color{orange}{(F: #1)}}}
\def\tomnote#1{{\color{cyan}{(Tom: #1)}}}
\def\mathnote#1{{\color{red}{(#1)}}}
\def\textnote#1{{\color{blue}{(#1)}}}
\def\companion#1{{\color{magenta}{(#1)}}}
\def\obsolete#1{{\color{brown}{#1}}}

%\usepackage{pdfcomment}
%\usepackage[color]{changebar}
%\cbcolor{red}
%\usepackage{bm}
%\usepackage{subfiles}

\usepackage[left=1in,top=1in,right=1in,bottom=1in]{geometry}
%\usepackage[left=1.5in,top=1.5in,right=1.5in,bottom=1.4in]{geometry}

%\linespread{1.1}     %this works nicely to produce a more readable cropped 2-1
\usepackage{scalerel}    %%%%  used first for scaling \bullet  
\usepackage{stmaryrd}   %%%% for integer interval notation 
\usepackage{mathabx}   %% made \widecheck work  
\usepackage{hyphenat}
\usepackage{scalerel}    %%%%  used first for scaling \bullet  


\addtolength\marginparwidth{-0.4in}


\newcommand{\be}{\begin{equation}}
\newcommand{\ee}{\end{equation}}


\newtheorem{theorem}{Theorem}[section]
\newtheorem{lemma}[theorem]{Lemma}
\newtheorem{proposition}[theorem]{Proposition}
\newtheorem{corollary}[theorem]{Corollary}
\newtheorem{formal}[theorem]{Critical point derivation}
\newtheorem{experiment}[theorem]{Experimental Result}
\newtheorem{claim}[theorem]{Claim}
\newtheorem{problem}{Open Problem}
\newtheorem{problems}[problem]{Open Problems}

\theoremstyle{definition}
\newtheorem{definition}[theorem]{Definition}
\newtheorem{example}[theorem]{Example}
%\newtheorem{xca}[theorem]{Exercise}
\newtheorem{exercise}[theorem]{Exercise}
\newtheorem{assumption}[theorem]{Assumption}
\newtheorem{conj}[theorem]{Conjecture}

\theoremstyle{remark}
\newtheorem{remark}[theorem]{Remark}
\newenvironment{remarks}{\begin{remark}\normalfont}{\end{remark}}
\newtheorem{quest}{Question}


%\allowdisplaybreaks[1]
\allowdisplaybreaks[3]
%\allowdisplaybreaks  %broke up a lot of displays 


\numberwithin{figure}{section}
\numberwithin{equation}{section}



\definecolor{sussexg}{rgb}{0,0.7,0.7}
\definecolor{sussexp}{rgb}{0.4,0,0.4}
\definecolor{sussexb}{rgb}{0.4,0.4,0.7}
\definecolor{mygray}{rgb}{0.75,0.75,0.75}
\newcommand{\flint}[1]{[\![{#1}]\!]} 
%\newcommand{\eqcl}[1]{\langle{#1}\rangle}       
\newcommand{\eqcl}[1]{[{#1}]} 
\newcommand{\bggeqcl}[1]{\biggl[{#1}\biggr]} 
\newcommand{\clf}{{\mathbf f}}
\newcommand{\clg}{{\mathbf g}}    \newcommand{\clh}{{\mathbf h}}  
\newcommand{\fpath}{{\clf_\bbullet}}
\newcommand{\Sols}{{\mathbf S}}
\newcommand{\Solk}{{\mathbf K}}

\renewcommand{\P}{\mathbb{P}}
\newcommand{\E}{\mathbb{E}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\Q}{\mathbb{Q}}

\newcommand{\bfP}{\mathbf{P}}
\newcommand{\bfE}{\mathbf{E}}
\DeclareMathOperator{\BM}{P}

\newcommand{\cC}{\mathcal{C}}
\newcommand{\cN}{\mathcal{N}}
\newcommand{\cZ}{\mathcal{Z}}

\newcommand{\fbar}{\bar f}

\providecommand{\abs}[1]{\vert#1\vert}
\providecommand{\babs}[1]{\bigl\vert#1\bigr\vert}
\newcommand{\fl}[1]{\lfloor{#1}\rfloor} 


\newcommand{\Rnz}{\R_{*}}%Non-zero real numbers.

\newcommand{\Paths}{\cG}
\newcommand{\e}{\varepsilon}
\newcommand{\KPZ}{h}
\newcommand{\She}{Z}
\newcommand{\coShe}{Z}   %collective version of \She 
\newcommand{\Sheb}{Z_{\beta}}
\newcommand{\KPZb}{h_\beta}
\newcommand{\SBEb}{u_\beta}
\newcommand{\Stat}{U}
\newcommand{\wZ}{{\overline\w}}
\newcommand{\OmZ}{{\overline\Omega}}
\newcommand{\PZ}{{\overline\P}}
\newcommand{\filZ}{{\overline\sF}}
\newcommand{\Shenorm}{\mathcal Z}
\newcommand{\Shetemp}{\widetilde Z}
\newcommand{\rnShe}{\sZ}
\newcommand{\Glob}{u}
\newcommand{\rnSheb}{\sZ_{\beta}}
\newcommand{\Bus}{b}
\newcommand{\Poly}{Q}
\newcommand{\Polyb}{Q^\beta}
\newcommand{\PolyBus}{\mathbf Q}
\newcommand{\Polypp}{\mathbf Q}
\newcommand{\Polycouple}{{\overline{\mathbf Q}}}
\newcommand{\Xtmp}{\overline X}
\newcommand{\pcouple}{{\mathbf p}}
\newcommand{\heat}{\rho}
\newcommand\Mom[2]{D_{#1,#2}} %Supremum of moments of the solution to the SHE.
\newcommand\Mob[3]{D_{#1,#2,#3}} %Supremum of moments of the solution to the SHE with beta.
\DeclareMathOperator\supp{supp} %Support
\newcommand\what{\widehat\w}

\DeclareMathOperator\oE{E} %Upright E for the polymer/bridge expectations


%%%%
\newcommand\std{\leq_{st}}%Stochastic domination.


%%%DLR STUFF
 \def\DLR{\mathrm{DLR}} %DLR measures
\newcommand{\sifDLR}{\overrightarrow{\DLR}} %Semi-infinite forward DLR
\newcommand{\sibDLR}{\overleftarrow{\DLR}} %Semi-infinite backward DLR
\newcommand{\biDLR}{\overleftrightarrow{\DLR}} %Bi-infinite DLR
\DeclareMathOperator\co{co}%Convex hull
\DeclareMathOperator\ext{ext}%extreme points


%%The shifts appearing in the SPDE paper.
\DeclareMathOperator\Id{Id}%Notation for the identity transformation
\DeclareMathOperator\oT{T} %Notation for the translation
\newcommand{\shiftf}[2]{\oT_{#1,#2}} %shift on function space
\newcommand\shiftd[2]{\sT_{\!\!#1,#2}} %shift on distribution space
\newcommand\shiftp{\theta} %shift on the path space
\newcommand\shiftx{\tau} %spatial shift on the space of initial conditions
\DeclareMathOperator\reff{R} %reflection on function space
\newcommand\refd{\sR} %reflection on distribution space
\DeclareMathOperator\oS{S} %Notation for the shear transformation
\DeclareMathOperator\oD{D} %Notation for the dilation transformation
\newcommand\shearf[2]{\oS_{#1,#2}} %shear on function space
\newcommand\sheard[2]{\sS_{#1,#2}} %shear on distribution space
\newcommand\dif[2]{\oD_{#1,#2}} %dilation on function space
\newcommand\did[2]{\sD_{#1,#2}} %dilation on distribution space
\DeclareMathOperator\oG{G} %A generic transformation on functions.
\newcommand\nef{\oN} %Negative map on L^2 function.
\newcommand\ned{\sN} %Negative map on distributions.
\DeclareMathOperator\oN{N} %A generic transformation on functions.

\newcommand{\cG}{\mathcal{G}}
\newcommand{\cA}{\mathcal{A}}
\newcommand{\cD}{\mathcal{D}}
\newcommand{\cE}{\mathcal{E}}
\newcommand{\cH}{\mathcal{H}}
\newcommand{\cI}{\mathcal{I}}
\newcommand{\cM}{\mathcal{M}}
\newcommand{\cB}{\mathcal{B}}
\newcommand{\cK}{\mathcal{K}}
\newcommand{\cT}{\mathcal{T}}
\newcommand{\cL}{\mathcal{L}}
\newcommand{\V}{\mathbb{V}}
\newcommand{\Phat}{\widehat{\mathbb{P}}}
\newcommand{\Ehat}{\widehat{\mathbb{E}}}
\newcommand{\bfPbar}{\overline{\mathbf{P}}}
\newcommand{\Z}{\mathbb{Z}}
\newcommand{\N}{\mathbb{N}}
\renewcommand{\S}{\mathbb{S}}
\newcommand{\X}{\mathbb{X}}
\newcommand{\Y}{\mathbb{Y}}
\newcommand{\T}{\mathbb{T}}
\newcommand{\HHH}{\overline{\mathbb{H}}}
\newcommand{\cF}{\mathcal{F}}
\newcommand{\cX}{\mathcal{X}}
\newcommand{\cXx}{\mathcal{X}^x}
\newcommand{\kS}{\mathfrak{S}}
\newcommand{\ce}[1]{\lceil{#1}\rceil}
\def\Udense{\mathcal{D}}
\newcommand{\sig}{{\scaleobj{0.8}{\boxempty}}} 
\newcommand{\sigg}{{\scaleobj{0.9}{\boxempty}}} 
%\def\Bruno{\text{\Large$\curlywedge$}\hspace{-3pt}^\w}
\def\Bruno{\Lambda\hspace{-1pt}^\w}
\def\BrunoZ{\Lambda\hspace{-1pt}^\wZ}
\def\Brunohat{\Lambda\hspace{-1pt}^{\what}}
\def\viiva{\hspace{.7pt}\vert\hspace{.7pt}}
\def\bviiva{\hspace{.7pt}\big\vert\hspace{.7pt}}   %% big viiva, use with \She\bigl( ... \bviiva ... \bigr) 
\def\Bviiva{\hspace{.7pt}\Big\vert\hspace{.7pt}} 


\newcommand{\WW}{\mathbb{W}}
\newcommand{\HH}{\mathbb{H}}
\newcommand{\vv}{\lambda}

\DeclareMathOperator*{\esssup}{ess\,sup}
\DeclareMathOperator*{\essinf}{ess\,inf}

%%Specific sets 
\newcommand{\Sbset}{\mathcal{S}}
\newcommand{\Tbset}{\mathcal{T}}
\newcommand{\Vbset}{\mathcal{V}}
\def\InitMeas{{\mathcal M}}
\def\Cmeas{{L}}
\newcommand\varset{\overline{\bbR}_{{\scaleobj{0.8}{\uparrow}}}^4} %Parameter set (t,x,s,y)
\newcommand\varsets{\bbR_{{\scaleobj{0.8}{\uparrow}}}^4} %Strict parameter set (t,x,s,y)
\newcommand\varsett[2]{\overline{\bbR}_{{\scaleobj{0.8}{\uparrow}}}^4(#1,#2)} %Parameter set with truncations.
\newcommand\varsetts[2]{\bbR_{{\scaleobj{0.8}{\uparrow}}}^4(#1,#2)} %Parameter set with truncations.
\newcommand\varsetsg[3]{\bbR_{{\scaleobj{0.8}{\uparrow}}}^4(#1,#2,#3)} %Parameter set with truncations and a gap
\newcommand\varsetth{\bbR_{{\scaleobj{0.8}{\uparrow}}}^3} %Parameter set (t,x,s)
\newcommand\varsettw{\bbR_{{\scaleobj{0.8}{\uparrow}}}^2} %Parameter set (t,s)
\newcommand\varsetthg[3]{\bbR_{{\scaleobj{0.8}{\uparrow}}}^3(#1,#2,#3)} %Parameter set (t,x,s) restricted to t,s in (-#1,-#1), x in #(-#2,#2), and t-s\geq#3.
\DeclareMathOperator\loc{loc}
\newcommand\Init{{\mathbb F}}
%\newcommand\Radon{{\sM_+\!\cup\,\infimeas}}     original notation for \Radon 
\newcommand\radon{\overline\sM_{>0}}
\newcommand\MP{{\sM_{>0}}}
%\newcommand\Radon{{{\widetilde{\sM}_+^\infty}}
\newcommand\Radon{{\,{\widetilde{\!\sM}}}}
\newcommand\dradon{d_{\radon}}    %%%% the metric on \radon that includes the crazy identically infinite measure  
\newcommand\dRadon{d_{\Radon}}    %%%% the metric on \Radon
\newcommand\dCICP{d_{\CICP}}    %%%% the metric on \Radon
\newcommand\nCICP{{\Cadon^{\,n}_{{\scriptscriptstyle\textrm{HE}}}}}    %Cartesian product 
\newcommand\dtICP{d}    %%%% the metric on \Radon
\newcommand\ICM{\sM_{{\scriptscriptstyle\textrm{HE}}}} %Admissible initial condition measure set.
\newcommand\CICM{\sC_{{\scriptscriptstyle\textrm{HE}}}} %Admissible initial condition measure set.
\newcommand\nCICM{\sC^n_{{\scriptscriptstyle\textrm{HE}}}} %Cartesian product 
\newcommand\ICP{\sI_{>0}} %Admissible initial condition measure set.
\newcommand\wtICM{{\widetilde\sI}_{\sM}} %Admissible initial condition measure set.
%\newcommand\tICP{{\widetilde\sI}} 
\newcommand\tICP{{\Radon_{{\scriptscriptstyle\textrm{HE}}}}} 
\newcommand\Cadon{{\,{\widetilde{\!\sC}}}}
\newcommand\CICP{{\Cadon_{{\scriptscriptstyle\textrm{HE}}}}} 
\newcommand\CICPOm{{\Cadon^{\,\Omega}_{{\scriptscriptstyle\textrm{HE}}}}} 
%\newcommand\tICPc{{\widetilde\sI}_{\mathrm{cont}}} 
\newcommand\tICPc{{\Radon_{{\scriptscriptstyle\textrm{HE}},{\mathrm{cont}}}}} 
\newcommand\tICPla{{\Radon_{{\scriptscriptstyle\textrm{HE}},{\lambda}}}} 
\newcommand\wtBc{\wt B_{\mathrm{cont}}} 
\newcommand\ICexp{\sI_{\mathrm{exp}}} %Admissible initial condition measure set.
\newcommand\ICMM{\sI_{\sM,\sM}} %Admissible initial condition measure set.
\newcommand\ICR{\sI_{\sM^*}} %Admissible initial condition measure set.
\newcommand\ICF{\sI_f} %Admissible initial condition function set.

\newcommand\CKPZ{\sC_{{\scriptscriptstyle\textrm{KPZ}}}} %Admissible initial condition measure set for KPZ.
\newcommand\nCKPZ{{\sC^{\,n}_{{\scriptscriptstyle\textrm{KPZ}}}}}    %Cartesian product 
\newcommand\CKPZt{{\wt\sC}_{{\scriptscriptstyle\textrm{KPZ}}}} %Admissible initial condition measure set for KPZ.
\newcommand\nCKPZt{{\sC^{\,n}_{{\scriptscriptstyle\textrm{KPZ}}}}}    %Cartesian product 


\newcommand\timefun[2]{\sL_{#1,#2}} %L^2 closure of functions supported on the time interval (#1,#2)
\newcommand\fil{\sF^W} %Usual conditions filtration of the white noise
\newcommand\filhat{{\widehat\sF}^W} %Usual conditions filtration of the white noise
\newcommand\filt[1]{\sF^{#1}} %Filtration with a parameter for the exponent. This gets used to define the filtration that will be completed.
\newcommand\filthat[1]{{\widehat\sF}^{#1}} %Filtration with a parameter for the exponent. This gets used to define the filtration that will be completed.
\newcommand\cfil{\sG} %The filtration on the space of continuous functions.
\newcommand\nulls{\mathfrak{N}} %The \bbP nullsets.
\DeclareMathOperator\oQ{Q}
\newcommand{\CDP}{Q}
\newcommand{\tdist}{\sS'}
\newcommand{\meas}{\mu}
\newcommand{\piMP}{\pi}
\newcommand{\PMPinit}{P}
\newcommand{\PMP}{\Pi_{\PMPinit}}     %% drop the little  \pi from the path measure 
%\newcommand{\PMP}{\Pi_{\PMPinit,\piMP}}

%%Events in the poylmer proofs
\DeclareMathOperator\cyl{Cyl}


\DeclareMathOperator{\bD}{\mathbb{D}}


\DeclareMathOperator{\bbA}{\mathbb{A}}
\DeclareMathOperator{\bbB}{\mathbb{B}}
\DeclareMathOperator{\bbC}{\mathbb{C}}
\DeclareMathOperator{\bbD}{\mathbb{D}}
\DeclareMathOperator{\bbE}{\mathbb{E}}
\DeclareMathOperator{\bbF}{\mathbb{F}}
\DeclareMathOperator{\bbG}{\mathbb{G}}
\DeclareMathOperator{\bbH}{\mathbb{H}}
\DeclareMathOperator{\bbI}{\mathbb{I}}
\DeclareMathOperator{\bbJ}{\mathbb{J}}
\DeclareMathOperator{\bbK}{\mathbb{K}}
\DeclareMathOperator{\bbL}{\mathbb{L}}
\DeclareMathOperator{\bbM}{\mathbb{M}}
\DeclareMathOperator{\bbN}{\mathbb{N}}
\DeclareMathOperator{\bbO}{\mathbb{O}}
\DeclareMathOperator{\bbP}{\mathbb{P}}
\DeclareMathOperator{\bbQ}{\mathbb{Q}}
\DeclareMathOperator{\bbR}{\mathbb{R}}
\DeclareMathOperator{\bbS}{\mathbb{S}}
\DeclareMathOperator{\bbT}{\mathbb{T}}
\DeclareMathOperator{\bbU}{\mathbb{U}}
\DeclareMathOperator{\bbV}{\mathbb{V}}
\DeclareMathOperator{\bbW}{\mathbb{W}}
\DeclareMathOperator{\bbX}{\mathbb{X}}
\DeclareMathOperator{\bbY}{\mathbb{Y}}
\DeclareMathOperator{\bbZ}{\mathbb{Z}}

%bold face
\DeclareMathOperator{\bfA}{\mathbf{A}}
\DeclareMathOperator{\bfB}{\mathbf{B}}
\DeclareMathOperator{\bfC}{\mathbf{C}}
\DeclareMathOperator{\bfD}{\mathbf{D}}
\DeclareMathOperator{\bfF}{\mathbf{F}}
\DeclareMathOperator{\bfG}{\mathbf{G}}
\DeclareMathOperator{\bfH}{\mathbf{H}}
\DeclareMathOperator{\bfI}{\mathbf{I}}
\DeclareMathOperator{\bfJ}{\mathbf{J}}
\DeclareMathOperator{\bfK}{\mathbf{K}}
\DeclareMathOperator{\bfL}{\mathbf{L}}
\DeclareMathOperator{\bfM}{\mathbf{M}}
\DeclareMathOperator{\bfN}{\mathbf{N}}
\DeclareMathOperator{\bfO}{\mathbf{O}}
\DeclareMathOperator{\bfQ}{\mathbf{Q}}
\DeclareMathOperator{\bfR}{\mathbf{R}}
\DeclareMathOperator{\bfS}{\mathbf{S}}
\DeclareMathOperator{\bfT}{\mathbf{T}}
\DeclareMathOperator{\bfU}{\mathbf{U}}
\DeclareMathOperator{\bfV}{\mathbf{V}}
\DeclareMathOperator{\bfW}{\mathbf{W}}
\DeclareMathOperator{\bfX}{\mathbf{X}}
\DeclareMathOperator{\bfY}{\mathbf{Y}}
\DeclareMathOperator{\bfZ}{\mathbf{Z}}

\DeclareMathOperator{\bfa}{\mathbf{a}}
\DeclareMathOperator{\bfb}{\mathbf{b}}
\DeclareMathOperator{\bfc}{\mathbf{c}}
\DeclareMathOperator{\bfd}{\mathbf{d}}
\DeclareMathOperator{\bfe}{\mathbf{e}}
\def\bff{\mathbf{f}}
\DeclareMathOperator{\bfg}{\mathbf{g}}
\DeclareMathOperator{\bfh}{\mathbf{h}}
\DeclareMathOperator{\bfi}{\mathbf{i}}
\DeclareMathOperator{\bfj}{\mathbf{j}}
\DeclareMathOperator{\bfk}{\mathbf{k}}
\DeclareMathOperator{\bfl}{\mathbf{l}}
\DeclareMathOperator{\bfm}{\mathbf{m}}
\DeclareMathOperator{\bfn}{\mathbf{n}}
\DeclareMathOperator{\bfo}{\mathbf{o}}
\DeclareMathOperator{\bfp}{\mathbf{p}}
\DeclareMathOperator{\bfq}{\mathbf{q}}
\DeclareMathOperator{\bfr}{\mathbf{r}}
\DeclareMathOperator{\bfs}{\mathbf{s}}
\DeclareMathOperator{\bft}{\mathbf{t}}
\DeclareMathOperator{\bfu}{\mathbf{u}}
\DeclareMathOperator{\bfv}{\mathbf{v}}
\DeclareMathOperator{\bfw}{\mathbf{w}}
\DeclareMathOperator{\bfx}{\mathbf{x}}
\DeclareMathOperator{\bfy}{\mathbf{y}}
\DeclareMathOperator{\bfz}{\mathbf{z}}

\DeclareMathOperator{\bf0}{\mathbf{0}}

\DeclareMathOperator{\mfa}{\mathfrak{a}}
\DeclareMathOperator{\mfb}{\mathfrak{b}}
\DeclareMathOperator{\mfc}{\mathfrak{c}}
\DeclareMathOperator{\mfd}{\mathfrak{d}}
\DeclareMathOperator{\mfe}{\mathfrak{e}}
\DeclareMathOperator{\mff}{\mathfrak{f}}
\DeclareMathOperator{\mfg}{\mathfrak{g}}
\DeclareMathOperator{\mfh}{\mathfrak{h}}
\DeclareMathOperator{\mfi}{\mathfrak{i}}
\DeclareMathOperator{\mfj}{\mathfrak{j}}
\DeclareMathOperator{\mfk}{\mathfrak{k}}
\DeclareMathOperator{\mfl}{\mathfrak{l}}
\DeclareMathOperator{\mfm}{\mathfrak{m}}
\DeclareMathOperator{\mfn}{\mathfrak{n}}
\DeclareMathOperator{\mfo}{\mathfrak{o}}
\DeclareMathOperator{\mfp}{\mathfrak{p}}
\DeclareMathOperator{\mfq}{\mathfrak{q}}
\DeclareMathOperator{\mfr}{\mathfrak{r}}
\DeclareMathOperator{\mfs}{\mathfrak{s}}
\DeclareMathOperator{\mft}{\mathfrak{t}}
\DeclareMathOperator{\mfu}{\mathfrak{u}}
\DeclareMathOperator{\mfv}{\mathfrak{v}}
\DeclareMathOperator{\mfw}{\mathfrak{w}}
\DeclareMathOperator{\mfx}{\mathfrak{x}}
\DeclareMathOperator{\mfy}{\mathfrak{y}}
\DeclareMathOperator{\mfz}{\mathfrak{z}}
\DeclareMathOperator{\mfG}{\mathfrak{G}}
\DeclareMathOperator{\mfS}{\mathfrak{S}}

%script
\DeclareMathOperator{\sA}{\mathcal{A}}
\DeclareMathOperator{\sB}{\mathcal{B}}
\DeclareMathOperator{\sC}{\mathcal{C}}
\DeclareMathOperator{\sD}{\mathcal{D}}
\DeclareMathOperator{\sE}{\mathcal{E}}
\DeclareMathOperator{\sF}{\mathcal{F}}
\DeclareMathOperator{\sG}{\mathcal{G}}
\DeclareMathOperator{\sH}{\mathcal{H}}
\DeclareMathOperator{\sI}{\mathcal{I}}
\DeclareMathOperator{\sJ}{\mathcal{J}}
\DeclareMathOperator{\sK}{\mathcal{K}}
\DeclareMathOperator{\sL}{\mathcal{L}}
\DeclareMathOperator{\sM}{\mathcal{M}}
\DeclareMathOperator{\sN}{\mathcal{N}}
\DeclareMathOperator{\sO}{\mathcal{O}}
\DeclareMathOperator{\sP}{\mathcal{P}}
\DeclareMathOperator{\sQ}{\mathcal{Q}}
\DeclareMathOperator{\sR}{\mathcal{R}}
\DeclareMathOperator{\sS}{\mathcal{S}}
\DeclareMathOperator{\sT}{\mathcal{T}}
\DeclareMathOperator{\sU}{\mathcal{U}}
\DeclareMathOperator{\sV}{\mathcal{V}}
\DeclareMathOperator{\sW}{\mathcal{W}}
\DeclareMathOperator{\sX}{\mathcal{X}}
\DeclareMathOperator{\sY}{\mathcal{Y}}
\DeclareMathOperator{\sZ}{\mathcal{Z}}
%
%\DeclareMathOperator{\lc}{\lceil}
%\DeclareMathOperator{\rc}{\rceil}
%\DeclareMathOperator{\lf}{\lfloor}
%\DeclareMathOperator{\rf}{\rfloor}
%\DeclareMathOperator{\Var}{{\mathbb V}ar}
%\DeclareMathOperator{\esup}{\bbP-esssup}
%\DeclareMathOperator{\einf}{\bbP-essinf}
%\DeclareMathOperator{\supp}{supp}
%
%
%\def\Diff{\cD}
%\def\Cont{\cC}
\def\w{\omega}
%\def\wbar{{\bar\w}}
%\def\wtil{{\tilde\w}}
%\newcommand{\ehat}{\widehat{e}}
%\def\unif{\vartheta}
%\def\Unif{\Gamma}
%\def\eB{\kappa}
%\def\EB{\cK}
%\def\Bavg{\overline B}
%\def\Gbar{\overline G}
%\def\what{{\widehat\w}}
\def\Qbar{\overline Q}
 \def\wt{\widetilde}  \def\wh{\widehat} \def\wb{\overline}
 \def\wc{\widecheck}
\def\Omhat{\widehat\Omega}
\def\Ombar{\overline\Omega}
\def\cFhat{\widehat\cF}
%\def\ddd{\displaystyle}
%\def\fe{\Lambda}
%\def\fepl{\fe_{\rm{pl}}}
%\def\Zne{Z^{\rm NE}} 
%\def\Qne{Q^{\rm NE}} 
%\def\Zn{Z^{\rm N}} 
%\def\xibar{\bar\xi}
%\def\Abar{\overline A}
%\def\zetabar{\bar\zeta}
%\def\etabar{\bar\eta}
%\def\hu{{\underline h}}
%\def\ho{{\overline h}}
%\def\ximin{{\underline\xi}}
%\def\ximax{{\overline\xi}}
%\def\ximinmin{\underline{\underline\xi}}
%\def\ximaxmax{\overline{\overline\xi}}
%\def\etaminmin{\underline{\underline\eta}}
%\def\etamaxmax{\overline{\overline\eta}}
%\def\zetaminmin{\underline{\underline\zeta}}
%\def\zetamaxmax{\overline{\overline\zeta}}
%\def\etamin{{\underline\eta}}
%\def\etamax{{\overline\eta}}
%\def\zetamin{{\underline\zeta}}
%\def\zetamax{{\overline\zeta}}
\DeclareMathOperator{\ri}{ri}    %rel interior  
%\DeclareMathOperator{\ext}{ext}    %extremes 
%\DeclareMathOperator{\dist}{dist} 
%%\def\xuDLR{x^{u,{\rm{DLR}}}}
%\def\XDLR{\overline X^{\,x,\w}}
%\def\Xtree{\widehat X^{\,\zeta,\w}}
%\def\Xtreen{\widehat X^{\,\zeta,\w,(n)}}
%%\def\backpix{{\overleftarrow{\pi}}^x} 
%%\def\backpi{{\overset{\small\leftarrow}{\pi}}{}} 
%\def\DLR{\mathrm{DLR}}
%\newcommand{\siDLR}{\overrightarrow{\DLR}}
%\newcommand{\biDLR}{\overleftrightarrow{\DLR}}
%\def\CI{\phi}
%\def\cid{\xi_*}
%\def\pici{\pi^{\rm{cif}}}
%\def\ker{\kappa}
%%\def\cid{\xi^*}
%\def\Bci{B^*}
%\def\Bcil{B^{*,\text\rm{(l)}}}
%\def\Bcir{B^{*,\text\rm{(r)}}}
%\def\Bbar{\overline B}
%\def\Bbarci{\bar B^*}
%%\def\cidm{\cid}
%\def\cidmin{\underline\xi_{^{\scriptstyle*}}}
%\def\cidmax{\overline\xi_*}
%\def\ci{{\rm ci}}
%\def\Pibar{\overline\Pi}
%\def\Pici#1{\Pi^{\ci,\w,#1}}
%\def\Picil#1{\Pi^{\ci,\w,\text\rm{(l)},#1}}
%\def\Picir#1{\Pi^{\ci,\w,\text\rm{(r)},#1}}
%\def\picix{\pi^{x,\ci}}
%%\def\varphimin{\varphi^{{\text\rm{(l)}}}}
%%\def\varphimax{\varphi^{{\text\rm{(r)}}}}
%\def\cidl{\cid^{\text\rm{(l)}}}
%\def\cidr{\cid^{\text\rm{(r)}}}
%\def\cidlmin{\cidmin^{\text\rm{(l)}}}
%\def\cidrmin{\cidmin^{\text\rm{(r)}}}
%\def\cidlmax{\cidmax^{\text\rm{(l)}}}
%\def\cidrmax{\cidmax^{\text\rm{(r)}}}
%%\def\cTl{\cT^{\textrm{(l)}}}
%%\def\thetal{\theta_*^{\text\rm{(l)}}}
%%\def\thetar{\theta_*^{\text\rm{(r)}}}
%%\def\Bcir{\overline B_*}
%%\def\Bcil{\underline B_*}
%
%\newcommand{\That}{\widehat{T}}
%\def\Omtemphat{\widehat\Omega_0}
%\def\Ommono{\Omega_{\rm{coc}}} %the Omega on which monotonicity (and other properties?) of cocycles holds
%\def\Ommonohat{\widehat\Omega_{\rm{coc}}} %the Omega on which monotonicity (and other properties?) of cocycles holds
%\def\Omcont#1{\Omega_{\rm{cont},#1}} %the Omega on which continuity holds at \xi
%\def\Omconthat#1{\widehat\Omega_{\rm{cont},#1}} %the Omega on which continuity holds at \xi
%\def\Omconstt#1{\Omega_{\rm{tilt},#1}} %the Omega on which h(B) is constant
%\def\Omconsthat#1{\widehat\Omega_{\rm{tilt},#1}} %the Omega on which h(B) is constan
%\def\Omback#1{\Omega_{#1,\downarrow0}} %the Omega on which the B-tree dies out
%\def\OmBus{\Omega_{[\ximin,\ximax]}} %the Omega on which liminf and limsup bounds hold for Busemann limits for the given \xi
%\def\Ombi{\Omega_{\rm{bi},[\ximin,\ximax]}} %the Omega on which liminf and limsup bounds hold for Busemann limits for the given \xi
%\def\OmBuszeta{\Omega_{[\zetamin,\zetamax]}} %the Omega on which liminf and limsup bounds hold for Busemann limits for the given \zeta
%\def\OmBusnice{\Omega_1} %the Omega on which Busemann limits exist on a dense set
%\def\OmBusa{\Omega_a} %the Omega on which one force one solution holds 
%\def\Omshape{\Omega_{\rm{shape}}} %the Omega on which the shape thms hold
%\def\OmBushat{\widehat\Omega_{[\ximin,\ximax]}} %the Omega on which Busemann limit holds
%\def\OmBushatzeta{\widehat\Omega_{[\zetamin,\zetamax]}} %the Omega on which liminf and limsup bounds hold for Busemann limits 
%\def\OmBusallhat{\widehat\Omega_{\rm{Bus}}} %the Omega on which liminf and limsup bounds hold for Busemann limits for all \xi
%\def\OmBusall{\Omega_{\rm{Bus}}} %the Omega on which liminf and limsup bounds hold for Busemann limits for all \xi
%\def\Omexist{\Omega_{\rm{exist}}} %the Omega on which directedness of cocycle DLRs holds
%\def\Omexistxi{\Omega_{\rm{exist},\xi}} %the Omega on which directedness of cocycle DLRs holds
%\def\Omexisthat{\widehat\Omega_{\rm{exist}}} %the Omega on which directedness of cocycle DLRs holds
%\def\Omdir{\Omega_{\rm{dir}}} %the Omega on which every DLR is directed
%\def\Omdirhat{\widehat\Omega_{\rm{dir}}} %the Omega on which every DLR is directed
%\def\OmBusPi{\Omega'_{[\ximin,\ximax]}} %the Omega on which DLR is Busemann for the given \xi
%\def\OmBusPihat{\widehat\Omega'_{[\ximin,\ximax]}} %the Omega on which DLR is Busemann for the given \xi
%\def\OmBusPiall{\Omega_{\rm{uniq}}} %the Omega on which Busemann limits will hold for all directions at once
%\def\OmBusPiallhat{\widehat\Omega_{\rm{uniq}}} %the Omega on which Busemann limits will hold for all directions at once
%\def\Omnondeg{\Omega_{\rm{nondeg}}}  %the Omega on which the only non-degenerate DLR solutions are \Pi^{e_i}
%\def\OmBhat{\widehat\Omega_B}  %the Omega on which the DLR solution corresponding to B is directed
%%\def\OmB{\Omega_B}  %the Omega on which the DLR solution corresponding to B is directed
%\def\Omreg{\Omega_{\rm{reg}}} % the Omega on which regular conditional probabilities are supported on the projection
%\def\Omcif{\Omega_{\rm{cif}}} % the Omega on which regular conditional probabilities are supported on the projection
%\def\Omnonuniq{\Omega_{\rm{ex}}} %the Omega on which Usetnonuniq does not intersect linear segments and includes non-diff points
%\def\Omeihat{\widehat\Omega_{e_1,e_2}}
%
%
%\def\WLLN{WLLN$_\xi$}
%\def\SLLN{SLLN$_\xi$}
%\def\proj{\pi}
%\def\gDLR{\mathrm{gDLR}}
%\def\cgDLR{\mathrm{cgDLR}}
%
%
%
%\makeatletter
%\DeclareRobustCommand{\cev}[1]{%
%  \mathpalette\do@cev{#1}%
%}
%\newcommand{\do@cev}[2]{%
%  \fix@cev{#1}{+}%
%  \reflectbox{$\m@th#1\vec{\reflectbox{$\fix@cev{#1}{-}\m@th#1#2\fix@cev{#1}{+}$}}$}%
%  \fix@cev{#1}{-}%
%}
%\newcommand{\fix@cev}[2]{%
%  \ifx#1\displaystyle
%    \mkern#22mu
%  \else
%    \ifx#1\textstyle
%      \mkern#22mu
%    \else
%      \ifx#1\scriptstyle
%        \mkern#22mu
%      \else
%        \mkern#22mu
%      \fi
%    \fi
%  \fi
%}
%
%\makeatother
%
%\def\backpix{{\cev{\pi}}^{\,x}} 
%
%
%\def\esssup{\mathop{\mathrm{ess\,sup}}}
%\def\range{\mathcal R}
\def\Uset{\mathcal U}
%%\def\Usetnice{\Uset_1}
%\def\Usetnonuniq{\Uset_x^\w}
%\def\Usetnonuniqz{\Uset_0^\w}
%\def\Ddense{\Diff_0}
%\def\Usetnonuniqhat{\Uset_x^\what}
%%\def\riUset{\Uset^\circ}
%\def\initF{\mathbb F}
\def\initF{\mathbb F}
%\def\initFx{\mathbb F^{\mathrm{sp}}}
%
\font \mymathbb = bbold10 at 11pt
\newcommand{\one}{\mbox{\mymathbb{1}}}    %indicator function
\def\ind{\one} 
%
%
%
%%%\usepackage{hyphenat}
%%\newtheorem{thm}{Theorem}[section]
%%\newtheorem*{thm*}{Theorem}
%%\newtheorem{prop}[thm]{Proposition}
%%\newtheorem{lem}[thm]{Lemma}
%%\newtheorem{cor}[thm]{Corollary}
%%\newtheorem{co}[thm]{Corollary}
%%\newtheorem{cond}[thm]{Condition}
%%\newtheorem{de}[thm]{Definition}

\usepackage{filemod}

\overfullrule=5pt


%%%%%   Timo  %%%%%

\def\ddd{\displaystyle} 

\newcommand\aabullet{{\raisebox{1.3pt}{\hspace{0.6pt}\scaleobj{0.55}{\bullet}\hspace{0.75pt}}}}  %%%% smaller bullet to use inside functions, needed to raise it a little and put space around 
\newcommand\abullet{{\raisebox{0.9pt}{\scaleobj{0.5}{\bullet}}}}  %%%% smaller bullet to use inside functions 
\newcommand\bbullet{{\raisebox{0.5pt}{\scaleobj{0.5}{\bullet}}}} %% looks good for paths x_\bbullet 
\newcommand\brbullet{{\raisebox{-0.5pt}{\scaleobj{0.4}{\bullet}}}} %%  for subscript paths x_\brbullet   need negative raise 
\newcommand\cbullet{{\raisebox{0.5pt}{\scaleobj{0.5}{\bullet}}}}   %% Suitable in the exponent of a subscript 
\newcommand\acbullet{{\raisebox{0.6pt}{\hspace{0.6pt}\scaleobj{0.55}{\bullet}\hspace{0.75pt}}}}  %%%% suitable bullet for a function in a superscript, for example Busemann in exponent 

\newcommand\dbullet{{\scaleobj{0.6}{\bullet}}}   % same as \bbullet but without shift up

\newcommand\bcdot{{\scaleobj{1.8}{\cdot}}}
\newcommand\acdot{{\raisebox{-1pt}{\scaleobj{1.4}{\cdot}}}}  %%dot inside function 



\def\tmart{G}  %%  martingale 
\def\tmarta{M} 
\def\SheOp{\Pi} 
\def\shift{\theta} 
\def\deq{\overset{d}=} 
\def\dto{\overset{d}\to}
\def\dtoo{\overset{d}\longrightarrow}

\def\evec{\mathbf e} 
\def\zevec{\mathbf 0} 
\def\onevec{\mathbf 1} 

 \def\gvec{\mathbf{g}} \def\fvec{\mathbf{f}}
\def\hvec{\mathbf{h}}  \def\tvec{\mathbf{t}}
\def\xvec{\mathbf{x}}
\def\yvec{\mathbf{y}}
\def\zvec{\mathbf{z}}
\def\wvec{\mathbf{w}}
\def\Bvec{\mathbf{B}}
\def\Yvec{\mathbf{Y}}  \def\Zvec{\mathbf{Z}} \def\thvec{\boldsymbol{\theta}}

\def\tsp{\hspace{0.5pt}}  %this is sometimes a good spacing in formulas when \, is too large 
\def\tspa{\hspace{0.7pt}}
\def\tspb{\hspace{0.9pt}}
\def\tspc{\hspace{1.1pt}}

\def\OFP{(\Omega, \cF, P)}     \def\OGP{(\Omega, \cG, P)} \def\OSP{(\Omega, \kS, \P)}
\def\OFbP{(\Omega, \cF, \P)} 
\def\OSPTh{(\Omega, \kS, \P, \Theta)}

\newcommand{\nn}{\nonumber}
\providecommand{\abs}[1]{\vert#1\vert}
\providecommand{\norm}[1]{\Vert#1\Vert}
\providecommand{\bnorm}[1]{\bigl\Vert#1\bigr\Vert}
\providecommand{\pp}[1]{\langle#1\rangle}
\newcommand{\abrac}[2]{{\langle#1,#2\rangle}}

\newcommand{\lzb}{\llbracket}   %left Z bracket  
\newcommand{\rzb}{\rrbracket}   %right Z bracket 

\DeclareMathOperator*{\sgn}{sgn}

\def\constkc{A}     %K-C constant 
\def\aconstkc{\sigma}     %another K-C constant 
%\def\infimeas{\overline\infty}   %% infinity measure 
%\def\infimeas{\skull}   %% infinity measure 
\def\infimeas{\rip}   %% infinity measure 
\def\zeromeas{\overline0}   %% zero measure 

\def\indep{\  \;{\raisebox{-1.5pt}{\text{\begin{rotate}{90}$\models$\end{rotate}}}}\ \, }  %independent random variables 
\def\nindep{\ \ \,{\raisebox{-1.5pt}{\text{\begin{rotate}{90}$\nvDash$\end{rotate}}}}\ \, }   %not independent random variables 
\def\qedex{\hfill$\triangle$} 
\def\qedrm{\hfill$\triangle$} 

\def\trrho{\boldsymbol\rho}   %another transition probability  

\def\bbvar{g}   %% a generic function-valued variable  
\def\bbus{b}    %% macro for the "Busemann" that comes from the ergodic measure \PMPinit
\def\BBus{\Bus}   %%% alt. macro for the main Busemann function 
\def\GaBbfP{(\Gamma, \cB_\Gamma, \bfP)}   %% probability space 
\def\bShe{\She}  %coordinate variable on a function space 

\def\Xsvelo{\overline\chi}  %limsup of X_r/r  X sup velocity   
\def\Xivelo{\underline\chi}  %liminf of X_r/r  X inf velocity 
\def\Xvelo{\chi}  %limsup of X_r/r  X sup velocity  

\def\PMPslopep{\overline\kappa}     %% PMP slope plus 
\def\PMPslopem{\underline\kappa}  %% PMP slope minus 

\newcommand\ttset{\mathscr{T}} 
%%%%%   end Timo %%%%%

